Modeling the Background for Incremental and Weakly-Supervised Semantic Segmentation

Deep neural networks have enabled major progresses in semantic segmentation. However, even the most advanced neural architectures suffer from important limitations. First, they are vulnerable to catastrophic forgetting, i.e. they perform poorly when they are required to incrementally update their model as new classes are available. Second, they rely on large amount of pixel-level annotations to produce accurate segmentation maps. To tackle these issues, we introduce a novel incremental class learning approach for semantic segmentation taking into account a peculiar aspect of this task: since each training step provides annotation only for a subset of all possible classes, pixels of the background class exhibit a semantic shift. Therefore, we revisit the traditional distillation paradigm by designing novel loss terms which explicitly account for the background shift. Additionally, we introduce a novel strategy to initialize classifier's parameters at each step in order to prevent biased predictions toward the background class. Finally, we demonstrate that our approach can be extended to point- and scribble-based weakly supervised segmentation, modeling the partial annotations to create priors for unlabeled pixels. We demonstrate the effectiveness of our approach with an extensive evaluation on the Pascal-VOC, ADE20K, and Cityscapes datasets, significantly outperforming state-of-the-art methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> cover_letter.tex <==
\onecolumn

\begin{coverletter}{Modeling the Background for Incremental and Weakly-Supervised Semantic Segmentation}{TPAMI-2020-10-1498}
 \begin{answereditor}{Reviewers agree on the importance of the task and on the quality of experimental results. However, they both express significant concerns that should be thoroughly addressed in a revised version of the manuscript.}{
We appreciate the reviewers' comments and suggestions. We have thoroughly revised the document accordingly, being certain that now it is substantially improved.
In relation to the writing, we clarified our contributions, and extended our discussion on weakly-supervised learning in the related works %
Moreover, we expanded our experimental analysis with the suggestions of reviewer 2, and the scribble-based weakly supervised setting, as suggested by reviewer 1. Without any modification to our method, it achieves results on par with the state of the art, showing that it is general and effective.
Below, we provide precise answers to the questions and issues raised by the reviewers, and we outline in green all the modifications introduced in the manuscript.}
 \end{answereditor}

\begin{answerreviewer}[Author Should Prepare A Major Revision For A Second Review]

\ca{In weakly supervised semantic segmentation, point-based supervision is actually very similar to the scribble-based supervision, which has been explored recently. It would be good if authors can include additional experiments on scribble-supervised semantic segmentation.}
{We thank the reviewer for the suggestion. In this revision, we include additional experiments on the scribble-supervised semantic segmentation setting in \refcm{exp:scribble}. 
The method and loss function proposed in our paper are general and can be applied also in the scribble context without any change. In particular, in Tab.~\ref{tab:scribble} we report the results our {weakly-supervised method (described in Section ~\ref{sec:weakly-met})} in the scribble supervised setting on the Pascal-VOC 2012 dataset \cite{lin2016scribblesup}. {The table confirms %
that exploiting priors on unlabeled pixels is crucial. %
In fact, our method %
obtains 72.3\% mIoU (75.1\% with CRF post-processing), outperforming the partial cross-entropy (PCE) baseline that applies the loss only on %
labeled pixels by a margin (69.5\% without and 72.8\% with CRF post-processing). Moreover, we note that our method with CRF post-processing is below the fully-supervised upper-bound only by 1.3\%, which is an outstanding result given the weak %
annotation. %
Compared to the state-of-the-art approaches specific for scribble-based segmentation \cite{lin2016scribblesup, tang2018normalized, tang2018regularized, wang2019boundary}, our method obtains comparable results. In particular, it achieves slightly lower performance than  NormalizedCut \cite{tang2018normalized} and KernelCut \cite{tang2018regularized} without using CRF post-processing (72.3\% ours, 72.8\% NormalizedCut, 73.0\% KernelCut) but achieves slightly superior results when using CRF (75.1\% ours, 74.5\% NormalizedCut, 75.0\% KernelCut). The results are expected since both NormalizedCut and KernelCut already exploit CRF during training, regularizing the model to output predictions consistent with the estimated object boundaries. This leads to better performances of these methods without CRF post-processing. %
Comparing our method with BPG \cite{wang2019boundary}, we see that the latter achieves 0.9\% more than MiB, both with and without CRF post-processing. However, BPG introduces two sub-networks in the segmentation architecture to model and improve the boundary predictions, largely increasing the number of parameters and requiring additional boundary supervision. Differently, our method does not change the network architecture and does not require additional supervision. %
} %
In conclusion, the results on the scribble-supervised setting demonstrate that our proposed method is general and can be adopted in multiple partially annotated settings without effort while achieving competitive results w.r.t. task-specific state-of-the-art models.
}

\ca{The authors should include more references on weakly-supervised semantic segmentation. It is helpful to improve the impact of this work.}{We thank the reviewer for the suggestion. %
We extended the related works on weakly supervised learning by considering not only point-based supervision, but also %
discussing approaches for image-level (\refcm{rel:weakly}) and scribble-based (\refcm{rel:weakly-scribble}).} %

\ca{This paper is an extended version of its earlier CVPR work. The newly added content mainly lies in the new experiments on the new task, i.e., point-supervised semantic segmentation, and one more dataset, i.e., Cityscapes. From my point, there are no new technical contributions.}
{%
In the CVPR version, we considered only the incremental learning scenario, identifying the background-shift problem and proposing a tailored solution for it using the priors %
we have on the semantic of unlabeled pixels.
In this extension, we show that the key idea of the proposed solution, \ie to use prior information on unlabeled pixels, is general and can be applied to any partially-supervised scenario. Differently from our previous version, we introduce the more general idea of modeling the uncertainty in Sec.~\ref{sec:method}. Then, we discuss its application in two special cases: incremental learning (Sec.~\ref{sec:incremental}, as in our CVPR paper), and weak supervision from either point-based or scribble-based supervision. %

{While this may appear a simple extension w.r.t the loss formulation, we argue that technical contribution is not trivial for two reasons: (i) we provide a new view of incremental learning for semantic segmentation associating the background-shift to the broader problem of learning from partial annotations, and (ii) we provide an elegant and general solution for learning from partial annotations that can be applied successfully in multiple settings with few or no changes, as demonstrated experimentally.}

In conclusion, we believe that the extended version may have a broader impact on the community since our methodological formulation is not limited to incremental learning but has a broader applicability. %
We clarified the contribution of the paper in \refcm{intro:novelty}.
}

\end{answerreviewer}


\vspace{1cm}
\begin{answerreviewer}[Author Should Prepare A Major Revision For A Second Review]

\ca{The authors should add a comparison to the complete-training baseline method in Table-1, Table-3, and Table-4. Specifically, the authors should train the segmentation model on the dataset with the complete category set for the same number of training epochs as the proposed method. I guess the proposed method requires a large number of training epochs. For example, for ADE20K experiments reported in Table-3, the authors should justify whether they train the model on the first 100 categories for 60 epochs and then 100+50 categories for another 60 epochs. If so, the authors should report the performance with the model trained over 150 categories for 120 epochs directly.}
{We apologize for the lack of clarity. The joint-training baselines, the upper bound of incremental learning methods, has been indeed trained for less epochs but it uses a larger dataset, resulting in approximately the same number of training iterations. For example, on the 100-50 setting of the ADE20K dataset, the joint training has been trained for nearly 50K iterations, while the incremental methods for 34K iterations on the initial step and 16K on the incremental one, \ie 50K iterations considering all steps.
Following the reviewer's suggestion, we performed the experiments using the same number of epochs as the incremental methods (resulting in more training iterations). %
We found that, on Pascal-VOC using 60 epochs hurts the performance, obtaining 76.5\% mIoU doubling the epochs, resulting in a decrease of 0.9\% mIoU \wrt the reported baseline (30 epochs). On ADE20K, using 120 epochs achieves a slight improvement, obtaining 39.3\% mIoU \wrt 38.9\% using 60 epochs. Finally, on Cityscapes the results are similar: using 360 epochs we obtain 73.1\% mIoU while using 720 slightly decreases the results by 0.3\%, resulting in 72.8\% mIoU. {Since the performance are comparable, we decided to be consistent and report the results at the same total number of iterations for all methods.}
}



\ca{The key insight of the transfer to point-supervised semantic segmentation is to treat the unlabeled pixels as the “incremental pixels” and apply supervision to constrain that the unlabeled pixels to one of the annotated classes with high probability. I guess that the authors apply a uniform probability vector over all annotated categories as the ground truth for all unlabeled pixels. Such an extension is very simple and seems not very related to the original incremental learning problem.}
{Extending the contribution of the previous paper, we investigated whether our approach for dealing with partial labels in incremental learning for segmentation can be extended to other partially-labeled scenarios, such as point supervision. In particular, we proposed a unified view of the two problems. Despite their differences, both incremental learning and point supervision have partial ground-truth annotations but they can impose priors on the unlabeled pixels. In incremental learning, we know that unlabeled pixels may be either background or any old class, while in point supervision %
all the unlabeled pixels belong to either a class in the set of point annotations or the background. 
In this work, we %
propose a general loss function that %
exploits semantic priors on unlabeled pixels in both settings, achieving results better than previous methods not using such inductive bias.%

We agree that the two tasks are not strictly related. However, we believe that the efficacy of our method in exploiting priors on unlabeled pixels in multiple scenarios is valuable. %
We clarified the technical contribution and the link between incremental learning and point-supervision in \refcm{intro:novelty}.
Finally, we remark that we are not forcing a uniform probability on the classes but we are forcing the sum of the probability of the classes in the prior to be one, as indicated in Eq.\eqref{eq:cases-ce}. A uniform distribution would force all the classes to have the same probability and, if a class is predicted with higher probability than others, it would be penalized. Differently, using Eq.\eqref{eq:cases-ce}, we {encourage the model to make predictions falling within the set of classes determined by the prior. This does not penalize high confidence prediction on any class of the set but only any probability assigned to classes not respecting the prior (\eg classes without any labeled pixel in point-supervision).} %
}

\ca{According to Table-5, surprisingly, such a simple additional supervision gains more than 6.5 mIoU score over PCT+bkg. The authors should provide a enhanced analysis on the reason of this large gap. Is the number of effective training samples the reason? If so, I guess you should train the PCT+bkg method with much longer iterations to achieve more fair comparisons as PCT+bkg only have very few effective training samples in each training iteration.}
{We argue that the benefits of MiB with respect PCE+bkg goes beyond the number of iterations. We performed the experiment suggested by the reviewer and we run the PCE+bkg baseline for 60 epochs, obtaining 37.6\% mIoU, which is 1.2\% below the result reported in the paper that was obtained using half of the epochs (30). 
The reason for the advantage of MiB \wrt PCE+bkg is on the type of training signal received from unlabeled pixels. In particular, both PCE+bkg and MiB use a 
partial cross-entropy (PCE) on the labeled pixels, as in Eq.\eqref{eq:unlabeled}. However, they handle differently the unlabeled ones: while in MiB we assume that unlabeled pixels may belong to any of the classes present in the annotation (\ie $\set{U}=\set{U}_x$), the PCE+bkg baseline considers them only as background (\ie $\set{U}$ only contains the background class). Thus, the PCE+bkg baseline is biased toward predicting the background class also on pixels belonging to foreground classes, leading to poor performances. {On the other hand, MiB allows the model to predict any of the annotated classes on unlabeled pixels, reducing the background bias and obtaining better results.}
We thank the reviewer and we revised the discussion of the result to clarify this aspect in \refcm{res:pcebkg}.
}

\ca{In both Table-5 and Table-6, the author should compare their method with more recent methods on the point-based weakly supervised scene parsing tasks.}
{We thank the reviewer for the suggestion. {We performed a deep literature search, also checking the bibliography of recent works in similar fields (\eg point-supervised object detection \cite{chen2021points} and instance segmentation \cite{cheng2021pointly}), but we did not find other more recent works (\wrt \cite{qian2019weakly}) performing point-based weakly supervised segmentation.} %
The 26 papers citing \cite{qian2019weakly} that we found (on Google Scholar in date September 6, 2021) either address a different task (\eg object detection, instance segmentation), or use different type of supervision. Thus, they are not comparable with the methods reported in Table 5 and 6.

}

\end{answerreviewer}

\end{coverletter}

 \twocolumn

